Preserving Automotive Heritage: A Blockchain-Based Solution for Secure Documentation of Classic Cars Restoration

Classic automobiles are an important part of the automotive industry and represent the historical and technological achievements of certain eras. However, to be considered masterpieces, they must be maintained in pristine condition or restored according to strict guidelines applied by expert services. Therefore, all data about restoration processes and other relevant information about these vehicles must be rigorously documented to ensure their verifiability and immutability. Here, we report on our ongoing research to adequately provide such capabilities to the classic car ecosystem. Using a design science research approach, we have developed a blockchain-based solution using Hyperledger Fabric that facilitates the proper recording of classic car information, restoration procedures applied, and all related documentation by ensuring that this data is immutable and trustworthy while promoting collaboration between interested parties. This solution was validated and received positive feedback from various entities in the classic car sector. The enhanced and secured documentation is expected to contribute to the digital transformation of the classic car sector, promote authenticity and trustworthiness, and ultimately increase the market value of classic cars.

==> sections/5_V_V.tex <==
\section{Evaluation}
\label{sec:v_and_v}

Evaluating the solution is crucial in a \gls{DSR} methodology. Therefore, it is vital to use precise and thorough methods to assess its impact, quality, and performance. 

\subsection{Performance Evaluation}

To assess the performance of our solution, our main focus centered on the \textit{ClassicsChain} Fabric application and \gls{API} through stress tests since this is the component that users will interact with. Users engage with it either through the \textit{ClassicsChain} front-end client or other clients invoking requests to our \gls{REST} \gls{API}.

Nevertheless, we also conducted evaluations of the individual performance of the Hyperledger Fabric blockchain network, our solution's cutting-edge technology. This assessment aimed to comprehend the unique performance characteristics of this component, gauge its impact on the overall system, and dissociate it from the performance of the Fabric application.

\subsubsection{Blockchain Network Evaluation}

For the individual blockchain network's performance evaluation, we employed \href{https://www.hyperledger.org/projects/caliper}{\textit{Hyperledger Caliper}} to analyze the performance through the invocation of various functions directly from the smart contracts deployed in the network.

The results from the tests using Caliper are displayed in \autoref{fig:caliper}. These results were obtained from evaluating the most up-to-date version of the blockchain network and smart contracts, allowing us to conclude the limits of our blockchain network in terms of supported \gls{TPS} for both read and write operations, clearly defining a maximum threshold for these operations. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=.7\linewidth]{figures/tps.png}
	\caption{Throughput results of our Hyperledger Fabric blockchain network.}
	\label{fig:caliper}
\end{figure}

We were able to determine the \gls{TPS} that our network supports, achieving a total of 70 TPS for read operations before the throughput decreases and a maximum of 22 TPS for write operations, beyond which the throughput significantly decreased and considerable failures were observed. No failures were noted in read operations.

Caliper also allows us to record latency duration in seconds. In typical network conditions and transaction send rates, we obtained average values of 0.16 seconds for read operations and 1.52 seconds for write operations.

\subsubsection{Fabric Application and API Evaluation}

Performance tests were conducted to simulate real users making requests using the Web app by employing Bash Shell scripts to communicate with the Web server via a REST API.

This evaluation aimed to determine the duration of the most important functionalities available through the respective endpoints. This assessment is essential as it evaluates the waiting time for end-users, from executing a specific request to obtaining the expected response, commonly referred to as load time.

\autoref{tab:performance} displays the minimum, average, and maximum duration times, in seconds, for the most frequently used requests, with each request being executed 30 times. Requests marked with an asterisk (*) refer to instances of that request with notable alterations, such as increased data to be uploaded or retrieved.

%\begin{scriptsize}

\begin{table}[]
\centering
\caption{Performance Evaluation: API request's duration, in seconds.}
\label{tab:performance}
\begin{tabular}{p{11cm}p{1cm}p{1cm}p{1cm}}
\hline
\rowcolor[HTML]{EFEFEF} 
\textbf{Request} & \textbf{Min.} & \textbf{Avg.} & \textbf{Max.} \\ \hline
1) Register a new user on the system & 0.81 & 0.93 & 1.28 \\
2) Login a user & 0.13 & 0.14 & 0.18 \\
3) Get the classic cars owned/authorized by a specific user (up to 30KB & 0.10 & 0.11 & 0.13 \\
3*) Get the classic cars owned/authorized by a specific user (up to 100KB) & 0.29 & 0.31 & 0.47 \\
4) Register a new classic car & 2.27 & 2.30 & 2.40 \\
5) Create a new restoration procedure (0 media files) & 2.29 & 2.32 & 2.38 \\
5*) Create a new restoration procedure (1 or 2 media files) & 2.37 & 2.42 & 2.70 \\
5**) Add a new restoration procedure (more than 5 media files) & 2.42 & 2.54 & 2.78 \\
6) Get the Vehicle Card of a specific classic (up to 50KB) & 0.09 & 0.10 & 0.10 \\
6*) Get the Vehicle Card of a specific classic (up to 100KB) & 0.25 & 0.26 & 0.30 \\
7) Get the History of the Vehicle Card of a specific classic (up to 50 KB) & 0.10 & 0.10 & 0.13 \\
7*) Get the History of the Vehicle Card of a specific classic (up to 300KB) & 0.36 & 0.43 & 0.45 \\
7**) Get the History of the Vehicle Card of a specific classic (2MB or more) & 6.27 & 8.40 & 12.14 \\
8) Grant/Revoke access permissions to a specific vehicle & 2.23 & 2.33 & 2.35 \\
9) Change a classic's owner & 2.21 & 2.46 & 2.7
\end{tabular}
\end{table}

%\end{scriptsize}


From the obtained results, write operations tend to be more consistent in terms of duration, as the volume of exchanged data remains fixed within an expected range. This consistency holds even when involving the upload of media files, thanks to the implementation of locally generating the \gls{CID}. However, some requests that read from the blockchain take longer when the volume of data to be received increases. For instance, when requesting the version history of a Vehicle Card with around 100 versions, such a query can take more than 12 seconds.

To conclude this performance evaluation, it is discernible that the request duration times for the functionalities within our solution are acceptable and reasonable within the context of blockchain-based systems and in the context of web applications for the classic car ecosystem. These durations offer users tolerable load times, ensuring a responsive experience. Upon analyzing all available requests, the average duration was calculated, obtaining an average of 2.5 seconds for write operations and 0.75 seconds for read functions, regardless of the data size being uploaded or retrieved. These duration values fall well within the acceptable threshold, remaining under the commonly tolerated 3-second waiting time for end-users in web systems, as proposed in \cite{nah2004study}.

\subsection{Relevance and Usability Evaluation}

Regarding the evaluation of our solution's relevance and the web application's usability, we followed a methodology based on questionnaires and interviews \cite{seidman2006interviewing}.

The participants in this evaluation included: one classic car owner; an automotive industry manager with extensive experience; the director of ACP Clássicos, a division within \gls{ACP} that certifies vehicles of historical interest; and both a business sales manager and commercial director from BASF, focusing on the BASF's Glasurit brand specialized in providing high-quality automotive coatings, used for refinishing classic car vehicles.

Initially, we presented a questionnaire on \textit{ClassicsChain} functionalities without revealing the ongoing solution. Responses supported the need for our work, indicating potential enhancements for existing classic automotive solutions.

Then, we explained how \textit{ClassicsChain} functions and demonstrated the majority of the features available in the web app. Furthermore, participants were given the chance to interact with the platform actively.

Following that, we used another questionnaire to evaluate the \gls{SUS} \cite{susArticle}. This questionnaire assessed the usability and user experience of the \textit{ClassicsChain} \gls{GUI}. The results of the questions can be consolidated into a total score. As each of the ten questions has 5 possible answers, these can be scored ranging from 0.0 to 10.0 with a 2.5 interval, resulting in a possible score for each question of 0.0, 2.5, 5.0, 7.5, or 10.0 depending on the tone of the question being positive or negative which alters the order of this sequence. By summing the values of all questions, a final score ranging from a minimum of 0.0 to a maximum of 100.0 is calculated. This cumulative value can then be better converted into a grade, ranging from A+ to F, or represented as a percentile \cite{susArticle}.

The participants' final scores in the \gls{SUS} section of the questionnaire are presented in \autoref{fig:susResults}. The average score yields a final result of 81, corresponding to a grade of A when converted. This score is considered above average for user experience and usability, surpassing the score of 80, as suggested by J. R. Lewis \cite{susArticle}.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=.7\linewidth]{figures/susResults.png}
	\caption{\gls{SUS} results for the \textit{ClassicsChain} web platform.}
	\label{fig:susResults}
\end{figure}

Additionally, we presented another questionnaire to gather opinions about the overall concept of the platform. The answers to these questions further emphasize the need for the work undertaken in this research and the relevance of \textit{ClassicsChain} and its distinctive features. Particularly noteworthy are the positive responses indicating participants' intentions to utilize the platform for future restoration procedures and their willingness to recommend it to other enthusiasts and entities involved in the classic automobile context.

\subsubsection{Threats to the Evaluation}

Upon completion of the relevance and usability assessment, it is important to clarify the validation threats identified. Moderator presence in interviews and questionnaires poses a validation threat, potentially biasing participant responses to please or displease the moderator and impact the research.

Moreover, due to time and availability constraints, the participant sample was restricted to five individuals, potentially affecting result precision.

Additionally, despite being unrelated to our work or the solution developed, some participants had prior exposure to the workshop where the solution was developed, which might introduce a positive bias in responses to maintain a favorable relationship.

Some participants could not explore the platform themselves. While all participants observed the platform in operation, mere observation might not suffice to evaluate certain usability aspects comprehensively. The absence of hands-on experience could have influenced the outcomes, potentially presenting outcomes that are either more favorable or less accurate. Additionally, participants used the interface in a controlled interview environment, impacting result authenticity compared to their natural interaction.
